SyntaxSQLNet: Syntax Tree Networks for Complex and Cross-DomainText-to-SQL Task

Most existing studies in text-to-SQL tasks do not require generating complex SQL queries with multiple clauses or sub-queries, and generalizing to new, unseen databases. In this paper we propose SyntaxSQLNet, a syntax tree network to address the complex and cross-domain text-to-SQL generation task. SyntaxSQLNet employs a SQL specific syntax tree-based decoder with SQL generation path history and table-aware column attention encoders. We evaluate SyntaxSQLNet on the Spider text-to-SQL task, which contains databases with multiple tables and complex SQL queries with multiple SQL clauses and nested queries. We use a database split setting where databases in the test set are unseen during training. Experimental results show that SyntaxSQLNet can handle a significantly greater number of complex SQL examples than prior work, outperforming the previous state-of-the-art model by 7.3% in exact matching accuracy. We also show that SyntaxSQLNet can further improve the performance by an additional 7.5% using a cross-domain augmentation method, resulting in a 14.8% improvement in total. To our knowledge, we are the first to study this complex and cross-domain text-to-SQL task.

==> old/results_table_anthology_ver.tex <==
\begin{table*}[ht!]
\centering
\scalebox{0.95}{
\begin{tabular}{lccccc}
\hline
 Method                         & Easy    & Medium  & Hard   & Extra Hard & All    \\ \hline
Seq2Seq                         & 17.9\% & 2.7\% & 1.3\% & 0.6\% & 5.4\% \\
Seq2Seq+Attention \cite{dong16} & 17.9\%  & 2.9\%   & 1.8\%  & 1.3\%      & 5.7\%  \\
Seq2Seq+Copying                 & 15.1\%  & 3.4\%	& 1.0\%	& 1.3\%	& 5.2\% \\
\newcite{iyer17}                & 7.9\%   & 2.1\%   & 1.3\%  & 1.1\%      & 3.1\%  \\
% Seq2SQL \cite{Zhong2017}        & 1.9\%   & 0.5\%   & 0.0\%  & 0.0\%      & 0.7\%  \\
SQLNet \cite{Xu2017}            & 23.7\%  & 5.9\%   & 2.3\%  & 0.3\%      & 8.3\%  \\
TypeSQL \cite{Yu18}             & 29.6\%  & 6.1\%   & 2.3\%  & 0.3\%      & 9.7\%  \\ \hline
SyntaxSQLNet	                & \textbf{43.1\%}  & \textbf{19.2\%}  & \textbf{17.8\%} & \textbf{4.8\%} & \textbf{22.0\%} \\
-augment	                    & 36.9\%  & 16.7\%  & 9.5\%  & 1.6\% & 17.6\%  \\
-wikiSQL -augment 
% & 36.5\%  &  12.8\%  & 11.0\% & 3.5\% &  16.3\%\\      
& 34.1\%  & 11.2\%  & 9.0\%  & 2.2\% & 14.5\% \\
-table -wikiSQL -augment 	    & 30.1\%  & 7.3\%   & 4.5\%  & 1.9\% & 10.9\% \\
-history -table -wikiSQL -augment   & 18.8\%  & 4.5\%	& 0.0\%	 & 0.0\%	  & 6.1\% \\
\hline
\end{tabular}}
\vspace{-2mm}
\caption{Exact match accuracy on SQL queries with different hardness levels.}
\label{tab:exact}
\vspace{-1mm}
\end{table*}

\begin{table*}[ht!]
\centering
\scalebox{0.95}{
\begin{tabular}{lcccccc}
\hline
 Method           & \texttt{SELECT} & \texttt{WHERE} & \texttt{GROUP BY} & \texttt{ORDER BY} & \texttt{KEYWORDS} \\\hline
Seq2Seq           & 13.7\% & 3.7\%  & 3.2\% & 4.9\% & 8.9\% \\
Seq2Seq+Attention & 14.0\%	& 5.0\%	& 3.2\%	& 6.1\%	& 9.4\% \\
Seq2Seq+Copying   & 12.0\%	& 2.7\%	& 5.2\%	& 6.9\%	& 6.7\% \\
\newcite{iyer17}  & 6.3\%	& 1.9\%	& 3.0\%	& 3.6\%	& 3.5\% \\
%Seq2SQL           & 0.052	& 1	    & 0.035	& 0.07	& 1	    & 0.219 \\
SQLNet            & 24.0\%	& 18.0\%  & 11.8\% &  47.1\%	& 61.9\% \\
TypeSQL           & 36.2\%	& 14.7\%  & 6.4\%	& 49.5\%	& 59.4\% \\ \hline
SyntaxSQLNet	    & \textbf{48.2\%}	& \textbf{31.6\%}	  & \textbf{28.9\%}	& \textbf{58.4\%}	& \textbf{68.9\%} \\
-augment	        & 45.3\%	& 29.2\%	  & 22.0\%	& 47.3\%	    & {67.5\%} \\
-wikiSQL -augment 
% & 40.4\%  & 25.1\% & 18.2\% & 52.9\% &  \textbf{69.5\%} \\
& 39.0\%	& 20.6\%	  & 17.1\%	& 50.2\%	& 65.8\% \\
-table -wikiSQL -augment 	    & 29.0\%	& 15.0\%	  & 13.1\%	& 45.5\%	    & 67.0\% \\
-history -table -wikiSQL -augment 	                    & 18.6\%	& 10.5\%	  & 4.1\%	& 30.0\%	    & 49.1\% \\
\hline
\end{tabular}}
\vspace{-2mm}
\caption{F1 scores of Component Matching on all SQL queries.}
\label{tab:results_component}
\vspace{-2mm}
\end{table*}




\iffalse
\begin{table*}[ht!]
\centering
\scalebox{0.95}{
\begin{tabular}{cccccc}
\hline
 Method                         & Easy    & Medium  & Hard   & Extra Hard & All    \\ \hline
Seq2Seq                         & 17.9\% & 2.7\% & 1.3\% & 0.6\% & 5.4\% \\
Seq2Seq+Attention \cite{dong16} & 17.9\%  & 2.9\%   & 1.8\%  & 1.3\%      & 5.7\%  \\
Seq2Seq+Copying                 & 15.1\%  & 3.4\%	& 1.0\%	& 1.3\%	& 5.2\% \\
\newcite{iyer17}                & 7.9\%   & 2.1\%   & 1.3\%  & 1.1\%      & 3.1\%  \\
% Seq2SQL \cite{Zhong2017}        & 1.9\%   & 0.5\%   & 0.0\%  & 0.0\%      & 0.7\%  \\
SQLNet \cite{Xu2017}            & 23.7\%  & 5.9\%   & 2.3\%  & 0.3\%      & 8.3\%  \\
TypeSQL \cite{Yu18}             & 29.6\%  & 6.1\%   & 2.3\%  & 0.3\%      & 9.7\%  \\ \hline
ours w/o HS	                    & 18.8\%  & 4.5\%	& 0.0\%	 & 0.0\%	  & 6.1\% \\
ours + part HS	                & 25.2\%  & 8.2\%   & 0.8\%  & 0.3\% & 9.4\% \\
ours + full HS w/o table	    & 24.7\%  & 6.1\%   & 1.3\%  & 0.3\% & 8.4\% \\
ours + full HS	                & 32.0\%  & 10.3\%  & 7.3\%  & 2.5\% & 13.3\% \\
ours + wiki + full HS	        & 29.4\%  & 13.2\%  & 3.3\%  & 0.3\% & 13.0\%  \\
ours + wiki + full HS + augment	& 40.3\%  & 15.5\%  & 15.3\% & 3.8\% & 19.2\% \\ \hline
\end{tabular}}
\vspace{-2mm}
\caption{Accuracy of Exact Matching on SQL queries for different hardness levels.}
\label{tab:results}
\vspace{-1mm}
\end{table*}

\begin{table*}[ht!]
\centering
\scalebox{0.9}{
\begin{tabular}{ccccccc}
\hline
 Method           & \texttt{SELECT} & \texttt{WHERE} & \texttt{GROUP BY} & \texttt{ORDER BY} & \texttt{KEYWORDS} \\\hline
Seq2Seq           & 13.7\% & 3.7\%  & 3.2\% & 4.9\% & 8.9\% \\
Seq2Seq+Attention & 14.0\%	& 5.0\%	& 3.2\%	& 6.1\%	& 9.4\% \\
Seq2Seq+Copying   & 12.0\%	& 2.7\%	& 5.2\%	& 6.9\%	& 6.7\% \\
\newcite{iyer17}  & 6.3\%	& 1.9\%	& 3.0\%	& 3.6\%	& 3.5\% \\
%Seq2SQL           & 0.052	& 1	    & 0.035	& 0.07	& 1	    & 0.219 \\
SQLNet            & 24.0\%	& 18.0\%  & 11.8\% &  47.1\%	& 61.9\% \\
TypeSQL           & 36.2\%	& 14.7\%  & 6.4\%	& 49.5\%	& 59.4\% \\ \hline
ours w/o HS	                    & 18.6\%	& 10.5\%	  & 4.1\%	& 100\%	    & 49.1\% \\
ours + part HS	                & 28.8\%	& 16.6\%	  & 10\%	& 100\%	    & 52.8\% \\
ours + full HS w/o table	    & 25.9\%	& 14.1\%	  & 8.1\%	& 100\%	    & 53.9\% \\
ours + full HS	                & 37.0\%	& 21.3\%	  & 15.2\%	& 47.8\%	& 68.1\% \\
ours + wiki + full HS	        & 36.4\%	& 29.4\%	  & 13.5\%	& 100\%	    & 56.4\% \\
ours + wiki + full HS + augment	& 44.9\%	& 28.3\%	  & 26.8\%	& 56.2\%	& 67.4\% \\\hline
\end{tabular}}
\vspace{-2mm}
\caption{F1 scores of Component Matching on all SQL queries.}
\label{tab:results_component}
\vspace{-3mm}
\end{table*}
\fi

==> old/results_table_init_submit.tex <==
\begin{table*}[ht!]
\centering
\scalebox{0.80}{
\begin{tabular}{lccccc}
\hline
 Method                         & Easy    & Medium  & Hard   & Extra Hard & All    \\ \hline
Seq2Seq                         & 17.9\% & 2.7\% & 1.3\% & 0.6\% & 5.4\% \\
Seq2Seq+Attention \cite{dong16} & 17.9\%  & 2.9\%   & 1.8\%  & 1.3\%      & 5.7\%  \\
Seq2Seq+Copying                 & 15.1\%  & 3.4\%	& 1.0\%	& 1.3\%	& 5.2\% \\
\newcite{iyer17}                & 7.9\%   & 2.1\%   & 1.3\%  & 1.1\%      & 3.1\%  \\
% Seq2SQL \cite{Zhong2017}        & 1.9\%   & 0.5\%   & 0.0\%  & 0.0\%      & 0.7\%  \\
SQLNet \cite{Xu2017}            & 23.7\%  & 5.9\%   & 2.3\%  & 0.3\%      & 8.3\%  \\
TypeSQL \cite{Yu18}             & 29.6\%  & 6.1\%   & 2.3\%  & 0.3\%      & 9.7\%  \\ \hline
SyntaxSQLNet	                & \textbf{40.3\%}  & \textbf{15.5\%}  & \textbf{15.3\%} & \textbf{3.8\%} & \textbf{19.2\%} \\
-augment	                    & 32.5\%  & 13.5\%  & 11.1\%  & 1.3\% & 15.6\%  \\
-wikiSQL -augment	                & 32.0\%  & 10.3\%  & 7.3\%  & 2.5\% & 13.3\% \\
-table -wikiSQL -augment 	    & 24.7\%  & 6.1\%   & 1.3\%  & 0.3\% & 8.4\% \\
-history -table -wikiSQL -augment   & 18.8\%  & 4.5\%	& 0.0\%	 & 0.0\%	  & 6.1\% \\
\hline
\end{tabular}}
\vspace{-2mm}
\caption{Exact match accuracy on SQL queries with different hardness levels.}
\label{tab:exact}
\vspace{-1mm}
\end{table*}

\begin{table*}[ht!]
\centering
\scalebox{0.80}{
\begin{tabular}{lcccccc}
\hline
 Method           & \texttt{SELECT} & \texttt{WHERE} & \texttt{GROUP BY} & \texttt{ORDER BY} & \texttt{KEYWORDS} \\\hline
Seq2Seq           & 13.7\% & 3.7\%  & 3.2\% & 4.9\% & 8.9\% \\
Seq2Seq+Attention & 14.0\%	& 5.0\%	& 3.2\%	& 6.1\%	& 9.4\% \\
Seq2Seq+Copying   & 12.0\%	& 2.7\%	& 5.2\%	& 6.9\%	& 6.7\% \\
\newcite{iyer17}  & 6.3\%	& 1.9\%	& 3.0\%	& 3.6\%	& 3.5\% \\
%Seq2SQL           & 0.052	& 1	    & 0.035	& 0.07	& 1	    & 0.219 \\
SQLNet            & 24.0\%	& 18.0\%  & 11.8\% &  47.1\%	& 61.9\% \\
TypeSQL           & 36.2\%	& 14.7\%  & 6.4\%	& 49.5\%	& 59.4\% \\ \hline
SyntaxSQLNet	    & \textbf{44.9\%}	& 28.3\%	  & \textbf{26.8\%}	& \textbf{56.2\%}	& 67.4\% \\
-augment	        & 42.1\%	& \textbf{28.4\%}	  & 21.9\%	& 47.2\%	    & \textbf{69.3\%} \\
-wikiSQL -augment	                & 37.0\%	& 21.3\%	  & 15.2\%	& 47.8\%	& 68.1\% \\
-table -wikiSQL -augment 	    & 23.1\%	& 11.4\%	  & 8.2\%	& 32.4\%	    & 51.7\% \\
-history -table -wikiSQL -augment 	                    & 18.6\%	& 10.5\%	  & 4.1\%	& 30.0\%	    & 49.1\% \\
\hline
\end{tabular}}
\vspace{-2mm}
\caption{F1 scores of Component Matching on all SQL queries.}
\label{tab:results_component}
\vspace{-3mm}
\end{table*}

\iffalse
\begin{table*}[ht!]
\centering
\scalebox{0.9}{
\begin{tabular}{cccccc}
\hline
 Method                         & Easy    & Medium  & Hard   & Extra Hard & All    \\ \hline
Seq2Seq                         & 17.9\% & 2.7\% & 1.3\% & 0.6\% & 5.4\% \\
Seq2Seq+Attention \cite{dong16} & 17.9\%  & 2.9\%   & 1.8\%  & 1.3\%      & 5.7\%  \\
Seq2Seq+Copying                 & 15.1\%  & 3.4\%	& 1.0\%	& 1.3\%	& 5.2\% \\
\newcite{iyer17}                & 7.9\%   & 2.1\%   & 1.3\%  & 1.1\%      & 3.1\%  \\
% Seq2SQL \cite{Zhong2017}        & 1.9\%   & 0.5\%   & 0.0\%  & 0.0\%      & 0.7\%  \\
SQLNet \cite{Xu2017}            & 23.7\%  & 5.9\%   & 2.3\%  & 0.3\%      & 8.3\%  \\
TypeSQL \cite{Yu18}             & 29.6\%  & 6.1\%   & 2.3\%  & 0.3\%      & 9.7\%  \\ \hline
ours w/o HS	                    & 18.8\%  & 4.5\%	& 0.0\%	 & 0.0\%	  & 6.1\% \\
ours + part HS	                & 25.2\%  & 8.2\%   & 0.8\%  & 0.3\% & 9.4\% \\
ours + full HS w/o table	    & 24.7\%  & 6.1\%   & 1.3\%  & 0.3\% & 8.4\% \\
ours + full HS	                & 32.0\%  & 10.3\%  & 7.3\%  & 2.5\% & 13.3\% \\
ours + wiki + full HS	        & 29.4\%  & 13.2\%  & 3.3\%  & 0.3\% & 13.0\%  \\
ours + wiki + full HS + augment	& 40.3\%  & 15.5\%  & 15.3\% & 3.8\% & 19.2\% \\ \hline
\end{tabular}}
\vspace{-2mm}
\caption{Accuracy of Exact Matching on SQL queries with different hardness levels.}
\label{tab:results}
\vspace{-1mm}
\end{table*}

\begin{table*}[ht!]
\centering
\scalebox{0.9}{
\begin{tabular}{ccccccc}
\hline
 Method           & \texttt{SELECT} & \texttt{WHERE} & \texttt{GROUP BY} & \texttt{ORDER BY} & \texttt{KEYWORDS} \\\hline
Seq2Seq           & 13.7\% & 3.7\%  & 3.2\% & 4.9\% & 8.9\% \\
Seq2Seq+Attention & 14.0\%	& 5.0\%	& 3.2\%	& 6.1\%	& 9.4\% \\
Seq2Seq+Copying   & 12.0\%	& 2.7\%	& 5.2\%	& 6.9\%	& 6.7\% \\
\newcite{iyer17}  & 6.3\%	& 1.9\%	& 3.0\%	& 3.6\%	& 3.5\% \\
%Seq2SQL           & 0.052	& 1	    & 0.035	& 0.07	& 1	    & 0.219 \\
SQLNet            & 24.0\%	& 18.0\%  & 11.8\% &  47.1\%	& 61.9\% \\
TypeSQL           & 36.2\%	& 14.7\%  & 6.4\%	& 49.5\%	& 59.4\% \\ \hline
ours w/o HS	                    & 18.6\%	& 10.5\%	  & 4.1\%	& 100\%	    & 49.1\% \\
ours + part HS	                & 28.8\%	& 16.6\%	  & 10\%	& 100\%	    & 52.8\% \\
ours + full HS w/o table	    & 25.9\%	& 14.1\%	  & 8.1\%	& 100\%	    & 53.9\% \\
ours + full HS	                & 37.0\%	& 21.3\%	  & 15.2\%	& 47.8\%	& 68.1\% \\
ours + wiki + full HS	        & 36.4\%	& 29.4\%	  & 13.5\%	& 100\%	    & 56.4\% \\
ours + wiki + full HS + augment	& 44.9\%	& 28.3\%	  & 26.8\%	& 56.2\%	& 67.4\% \\\hline
\end{tabular}}
\vspace{-2mm}
\caption{F1 scores of Component Matching on all SQL queries.}
\label{tab:results_component}
\vspace{-3mm}
\end{table*}
\fi

==> results_table_before_20181024.tex <==
\begin{table*}[ht!]
\centering
\scalebox{0.92}{
\begin{tabular}{l|ccccc|c}
\hline
\multirow{2}{*}{Method} & \multicolumn{5}{c|}{Test} & Dev \\ 
& Easy    & Medium  & Hard   & Extra Hard & All & All   \\ \hline
Seq2Seq                         & 17.3\% & 1.9\% & 1.3\% & 0.5\% & 4.9\% & 3.8\%  \\
Seq2Seq+Attention %\cite{dong16} 
& 18.1\% & 2.6\% & 2.0\% & 1.1\% & 5.6\% & 2.7\%   \\
Seq2Seq+Copying                 & 15.8\% & 3.4\% & 2.0\% & 1.1\% & 5.4\% & 4.1\%  \\
SQLNet %\cite{Xu2017}            
& 35.6\% & 13.3\% & 6.6\% & 1.3\% & 14.7\% & 14.3\%   \\
TypeSQL %\cite{Yu18}            
& 29.9\% & 7.6\% & 4.0\% & 0.8\% & 10.5\% & 10.6\%   \\ \hline   
SyntaxSQLNet	                & \textbf{61.2\%} & \textbf{28.1\%} & \textbf{26.9\%} & \textbf{5.1\%} & \textbf{31.1\%} &  \textbf{28.7\%} \\
-augment	                    & 50.3\%  & 18.6\% & 17.7\% & 4.9\%  & 23.0\% & 22.1\% \\
-table -augment & 49.5\% & 14.3\% & 13.2\% & 2.7\% &  19.7\% & 19.7\%\\
-history -table -augment ~~~  & 28.1\% & 7.3\% & 0.0\% & 0.0\%  & 9.1\% & 8.4\% \\
\hline
\end{tabular}}
\vspace{-2mm}
\caption{Accuracy of Exact Matching on SQL queries with different hardness levels.}
\label{tab:results}
\vspace{-1mm}
\end{table*}

\begin{table*}[ht!]
\centering
\scalebox{0.92}{
\begin{tabular}{lcccccc}
\hline
 Method           & \texttt{SELECT} & \texttt{WHERE} & \texttt{GROUP BY} & \texttt{ORDER BY} & \texttt{KEYWORDS} \\\hline
Seq2Seq           & 13.0\% & 1.5\% & 3.3\% & 5.3\% & 8.7\%  \\
Seq2Seq+Attention & 13.6\% & 3.1\% & 3.6\% & 9.9\% & 9.9\%  \\
Seq2Seq+Copying   & 12.0\% & 3.1\% & 5.3\% & 5.8\% & 7.3\%  \\
SQLNet            & 44.5\% & 19.8\% & 29.5\% & 48.8\% & 64.0\% \\
TypeSQL           & 36.4\% & 16.0\% & 17.2\% & 47.7\% & 66.2\% \\ \hline
SyntaxSQLNet      & \textbf{62.5\%} & \textbf{34.8\%} & \textbf{55.6\%} & \textbf{60.9\%} & 69.6\% \\
-augment	        & 53.9\% & 24.5\% & 44.4\% & 49.5\% & \textbf{71.3\%} \\
-table -augment 	    & 48.9\% & 20.1\% & 36.3\% & 46.8\% & 69.7\% \\
-history -table -augment ~~~	    & 26.7\%	& 14.6\%	  & 11.8\%	& 34.9\%	    & 64.6\% \\\hline
\end{tabular}}
\vspace{-2mm}
\caption{F1 scores of Component Matching on all SQL queries on Test set.}
\label{tab:results_component}
\vspace{-3mm}
\end{table*}
